Formal Analysis of Metastable Failures in Software Systems

Many large-scale software systems demonstrate metastable failures. In this class of failures, a stressor such as a temporary spike in workload causes the system performance to drop and, subsequently, the system performance continues to remain low even when the stressor is removed. These failures have been reported by many large corporations and considered to be a rare but catastrophic source of availability outages in cloud systems. In this paper, we provide the mathematical foundations of metastability in request-response server systems. We model such systems using a domain-specific language. We show how to construct continuous-time Markov chains (CTMCs) that approximate the semantics of the programs through modeling and data-driven calibration. We use the structure of the CTMC models to provide a visualization of the qualitative behavior of the model. The visualization is a surprisingly effective way to identify system parameterizations that cause a system to show metastable behaviors. We complement the qualitative analysis with quantitative predictions. We provide a formal notion of metastable behaviors based on escape probabilities, and show that metastable behaviors are related to the eigenvalue structure of the CTMC. Our characterization leads to algorithmic tools to predict recovery times in metastable models of server systems. We have implemented our technique in a tool for the modeling and analysis of server systems. Through models inspired by failures in real request-response systems, we show that our qualitative visual analysis captures and predicts many instances of metastability that were observed in the field in a matter of milliseconds. Our algorithms confirm that recovery times surge as the system parameters approach metastable modes in the dynamics.

==> discussion.tex <==
\subsection{Limitations: Model-System Mismatch}

Our CTMC model is an approximation of the precise operational model of a system.
For example, we ``average out'' timeouts and retries so that the average effect is maintained, but the distribution
of timeouts and retries may differ significantly from an operational model.
Further, owing to numerical issues, we approximate timeout computations using probability bounds.
We have used a discrete-event simulator to validate the fidelity of the CTMC model to an operational one.
Our experience is mixed.
When we simulate our model starting with an empty queue, we observe that the finite-time behavior of the CTMC (calculated by
solving the Kolmogorov equations) matches the corresponding values from simulation.
% (computed as the empirical means and variances over 100 runs).
However, the predictions from the CTMC model and the simulations differ---sometimes quite significantly---when we 
consider recovery times from full queues and large orbits for metastable configurations.
For example, \cref{fig:intro}(a) shows the queues do not clear after 600s in simulations, but the CTMC in \cref{fig:good_vs_bad_policy}
shows a 15\% reduction after 400s.
We expect these deviations, since our current modeling approximations are relatively coarse.
We leave a more precise modeling, and learning CTMCs from simulation data, as future work.

Nevertheless, we have found that our CTMC models and their predictions have strong exploratory and explanatory power.
In an industrial context, we have used the predictions of the CTMC as the starting point for more expensive simulation studies.

\begin{comment}
\paragraph{Numerical Approximations}
The computation of error probabilities and of hitting times in large CTMCs leads to numerical issues.
Thus, instead of exactly computing them, we often resort to numerical approximations, such as the use of Chebyshev inequalities to bound the error.
Moreover, when computing hitting times, we check the numerical precision of our solutions: since the system has high condition number,
the solutions can have large errors near metastability.
\end{comment}

==> metastability_theory.tex <==
\subsection{Formal Characterization of Metastability in CTMCs}\label{sec:ctmc_metastability}
%\paragraph{Metastability}
We now define metastability in a (finite) CTMC and provide a spectral characterization. First, we define the \emph{hitting time} for a set $D$ as the first (nonzero) time when the chain visits $D$, starting at some state $X(0)=x$:
\begin{equation}
 \label{eq:hitting_time}
  \tau_D = \inf \set{ t > 0 \mid X(t) \in D}. 
 \end{equation}
%
We could define metastability based on hitting times: a CTMC is metastable w.r.t.\ a set $D\subset S$ if
\begin{equation}\label{eq:metastability_def_ht}
|S|\frac{\sup_{x\not\in D} \mathbb{E}_x [\tau_D]}{\inf_{x\in D} \mathbb{E}_x [\tau_{D\setminus \set{x}}]} << 1,
\end{equation} 
that is, if the time scale of traveling between different states in $D$ is much larger than reaching some state in $D$.
However, in applications, we often want to \emph{predict} hitting times from a characterization of metastability, so this definition would be circular.
Following the analysis in \cite{BEGK2002,MetastabilityBook} for discrete time Markov chains, 
we provide an alternate definition in terms of escape probabilities.
For a state $x\in S$ and set $D\subset S$, define the \emph{escape probability} from $x$ to $D$ as $\prob_x(\tau_D<\tau_x)$.

\begin{definition}[Metastable sets]
	\label{def:metastability_def_v2}
	A finite CTMC $\M = (S, Q)$ is \emph{$\rho$-metastable with respect to a set $D \subset S$} if
	\begin{equation}
		\label{eq:meta_stability}
		|S| \frac{\sup _{x \in D} \mathbb{P}_x\left(\tau_{D \backslash x}<\tau_x\right)}{\inf _{y \notin D} \mathbb{P}_y\left(\tau_D<\tau_y\right)} \leq \rho \ll 1.
	\end{equation}
\end{definition}

Intuitively, a CTMC is $\rho$-metastable w.r.t.\ $D$ if the ratio of the largest escape time from a state in $D$ to a different state in $D$ to the smallest escape time from
any state outside of $D$ to $D$ is small; that is, any state in $D$ will visit a different state in $D$ at a time scale that is much larger than the time scale for it to visit itself
or the time scale for any state outside of $D$ to visit $D$.

While \cref{def:metastability_def_v2} defines metastability in terms of escape probabilities, computing escape probabilities in large CTMCs can be time consuming and numerically unstable. 
Therefore, we provide an alternate spectral characterization.
We need the following definition.

\begin{definition}[Nested subsets of metastable sets]
	\label{def:nested}
	%Definition 8.27 
	Let $D$ be a set of metastable points with $|D|=k$. Define the collection of sets $\{D_k,D_{k-1},\ldots,D_1\}$ inductively with $D_k=D$ and
	\begin{equation*}
		% \label{eq:nested}
		D_{\ell-1}:=D_{\ell} \backslash x_{\ell},\quad x_{\ell}:=\operatorname{argmax}_x\left[\mathbb{P}_x\left(\tau_{D_\ell \backslash x}<\tau_x\right), x \in D_{\ell}\right],\quad \forall\ell\in\{2,3,\ldots,k\},
	\end{equation*}
	The set $D$ is called \emph{non-degenerate} if for any $\ell\in\{1,2,\ldots,k\}$ the set $D_{\ell}$ is itself a set of metastable points.
\end{definition}

The following result is an extension of \cite[Theorem 8.43]{MetastabilityBook} for CTMCs and establishes a relation between 
metastability and the eigenvalues of the generator matrix $Q$.
While we state the theorem under the assumption of reversibility,
similar results hold for general non-reversible CTMCs (see \cite{eckhoff2002low}, Theorem~1.2). 
However, deriving these results without assumptions of reversibility requires additional machinery that goes beyond the scope of this paper and we omit these details. 

\begin{theorem}[Spectral Characterization]
\label{thm:hitting_time_spectral_rel}
	Let $\M = (S, Q)$ be an ergodic, reversible, finite CTMC.
	Assume $D\subset S$ is a metastable non-degenerate set, $|D| = k$, and the nested sets $\{D_1,\ldots,D_k\}$ constructed in Definition~\ref{def:nested} are also metastable with the same parameter $\rho$. 
	%
	Then %$-L = \mathbf{1} -P$ 
	% P = I+Q/E
	% Q = P-I = L
	$-Q$
	has $k$ eigenvalues $\lambda_1<\lambda_2<\cdots<\lambda_k$, where $\lambda_1=0$, and 	for some $\delta$ with $|S|\delta\leq\rho$, we have
	% %
	% \begin{equation*}
	% \lambda_{\ell}=\frac{\operatorname{cap}\left(x_{\ell}, D_{\ell-1}\right)}{\mu\left(A\left(x_{\ell}\right)\right)}[1+O(\delta)], \quad \ell=2, \ldots, k
	% \end{equation*}
	% %
	% Consequently,
	\begin{equation}\label{eq:eigenval_hitting_time}
		\lambda_{\ell}=\frac{1}{\mathbb{E}_{x_{\ell}}\left[\tau_{D_{\ell-1}}\right]}[1+O(\delta)]
		%=\frac{1}{\mathbb{E}_{x_{\ell}}\left[\tau_{D_{x_{\ell}}}\right]}[1+O(\delta)]
		,\quad \ell\in\{2,3,\ldots,k\}
	\end{equation}
	%where $D_{x_{\ell}} :=\{z\in D\,|\,\mu(z)> \mu(x_\ell)\}$.
	% The corresponding normalized eigenfunction has the form
	% \begin{equation*}
	% \psi_{\ell}(y)=\frac{h_{x_{\ell}, D_{\ell-1}}(y)}{\left\|h_{x_{\ell}, D_{\ell-1}}\right\|_{2, \mu}}+\sum_{j=1}^{\ell-1} O(\delta) \frac{h_{x_{\ell}, D_{j-1}}(y)}{\left\|h_{x_{\ell}, D_{j-1}}\right\|_{2,\mu}} .
	% \end{equation*}
\end{theorem}

Theorem~\ref{thm:hitting_time_spectral_rel} allows us to get estimates for metastable behavior and, through \cref{eq:eigenval_hitting_time}, estimates for hitting times,
through the computation of eigenvalues. 
This is useful in practice, since we can estimate the \emph{mixing time} for a chain using its eigenvalues. Informally, the mixing time measures how long the chain takes to reach its stationary distribution
and can be used as a proxy for hitting times.
(Hitting times are difficult to compute in a numerically stable way for metastable behaviors.)


%%The behaviors are stable or unstable, based on the ratio of arrival to service rates.  
% The hitting time from a full queue to an empty queue
% can be computed explicitly and is linear (in case of a stable queue) or exponential (unstable queue).
%This partly explains why a mathematical study of metastable modes is conspicuously absent in the queueing and probabilistic modeling literatures. \Mahmoud{I'm not sure if here is the right place for the above remark.}

\begin{remark}
We note that, although metastability has been extensively studied in the context of discrete-time Markov chains (DTMCs), a formal characterization for continuous-time Markov chains has been lacking. While the concept appears analogous across discrete and continuous-time frameworks, the underlying analysis and proofs differ significantly (see Sections~1.2 and 1.3 in the supplementary material).
\end{remark}

==> metastable.tex <==
\section{Metastability in Server Systems}\label{sec:CTMC_metastability}

Let $\M = (S, Q)$ be a CTMC and let $\piinf$ be its stationary distribution.
We denote the stationary probability assigned to a set $A\subset S$ by $\piinf(A)\coloneqq \sum_{i\in A}\piinf(i)$. 
We define the \emph{instantaneous escape rate} for a set $A\subset S$ as follows: 
\begin{equation}\label{eq:ration_def}
	\rho(A) = \sum_{i\in A}\piinf(i)\|\indic_i^\top Q\|_{\bar A},	
\end{equation}
where $\bar A=S\setminus A$, and $\indic_i$ is an indicator vector containing zero entries everywhere except at its $i$th entry where it has one,
and $|x|_{A} \coloneqq \sum_{i \in A} x_i$.

Let $\varepsilon, \delta \in [0, 1]$ be parameters and $m\geq 2$.
Assume $\M$ is an irreducible CTMC with stationary distribution $\piinf$.
A partition $(R_1, R_2, \ldots, R_m)$ of $S$ is called an $(\varepsilon, \delta)$-metastable partition of $\M$ if the following conditions hold:
	\begin{enumerate}
		\label{enum:metastable}
		\item $\rho(R_i)\le \epsilon$ and $\piinf(R_i) \geq \delta$ for all $i\in\set{1,\ldots,m}$. 
% and 
		% \item $\piinf(T)\leq\varepsilon$ and  $\rho(T)\geq\delta$.
	\end{enumerate}

Intuitively, $\varepsilon$ characterizes ``low'' probability and $\delta$ characterizes ``high'' probability.
The conditions state that each $R_i$ is assigned high occupancy by the stationary distribution but has small instantaneous escape rates.
% Moreover, the set $T$ has low occupancy but high escape rates.
In the long run, the chain will reside in the union of the $R_i$'s.
However, once it enters a specific $R_i$, it remains there for a long time before escaping to a different one.
We call the $R_i$s ``almost invariant'' sets: once in $R_i$, the escape out of it has a long expected time. 
% The set $T$ consists of the almost transient states that connect the $R_i$s to each other.
% \RM{omit $T$ altogether and only work with the recurrent states?}
We require $m\geq 2$: metastable behavior arises when there are multiple almost invariant sets. 


\RM{is there a way to compute bounds on hitting times using $\epsilon$ $\delta$ and $Q$?}


==> mm1_analysys.tex <==
We note that we can compute hitting times explicitly for M/M/c queues and their variants.
In particular, these systems do not show metastable behaviors.
We state the following theorem for M/M/1 queues, but similar results hold when $c>1$.

\begin{comment}
\begin{proposition}\label{prop:mm1_hitting_time}
For an M/M/1 queue characterized by the arrival rate $\lambda$, processing rate $\mu$, 
the expected time to hit a queue size $n$ from the current queue size $N>n$ is
\begin{equation}
    1.
\end{equation}
which is exponentially large with respect to $(N-n)$ for $\lambda>\mu$.

the expected time to hit a queue size $n$ from the current queue size $N<n$ is
\begin{equation}
    2.
\end{equation}
which is exponentially large with respect to $(n-N)$ for $\lambda<\mu$.

For the balanced case $\lambda = \mu$, the time to hit a queue size $n$ from queue size $N$ is
\begin{equation}
    3.
\end{equation}

and bounded queue size $N$, explicit form for expected time to drain a full queue is
\begin{equation}
\frac{N}{\mu-\lambda}+\lambda\frac{1-(\frac{\lambda}{\mu})^{N}}{(\mu-\lambda)^2}.
\end{equation}
\end{proposition}
\end{comment}

\begin{proposition}\label{prop:mm1_hitting_time}
\begin{comment}
For an M/M/1 queue characterized by the arrival rate $\lambda$, processing rate $\mu$, 
the expected time to hit a queue size $n$ from the current queue size $N>n$ is
\begin{equation}
    1.
\end{equation}
which is exponentially large with respect to $(N-n)$ for $\lambda>\mu$.

the expected time to hit a queue size $n$ from the current queue size $N<n$ is
\begin{equation}
    2.
\end{equation}
which is exponentially large with respect to $(n-N)$ for $\lambda<\mu$.

For the balanced case $\lambda = \mu$, the time to hit a queue size $n$ from queue size $N$ is
\begin{equation}
    3.
\end{equation}

and bounded queue size $N$, explicit form for expected time to drain a full queue is
\begin{equation}
\frac{N}{\mu-\lambda}+\lambda\frac{1-(\frac{\lambda}{\mu})^{N}}{(\mu-\lambda)^2}.
\end{equation}
\end{comment}
For an M/M/1 queue characterized by the arrival rate $\lambda$, processing rate $\mu$, and queue length $N$, 
the expected time to hit a queue size $0$ from the current queue size $i\in \nats$ takes the form
\begin{equation*}
\begin{cases}
    (A+Bi) + C\rho^ i & \rho \neq 1\\
    A+Bi+C i^2 & \rho = 1,
\end{cases}
\end{equation*}
where $\rho \coloneqq \frac{\lambda}{\mu}$, and $A, B, C$ are real numbers with $C\neq 0$.
\end{proposition}
\begin{proof}
	\begin{comment}
	Let us define $d_i$ to be the expected time to change the queue size from $i$ to $i-1$ for $i\geq 1$. We have 
	$$-d_i(\mu+\lambda)+(d_{i+1}+d_i)\lambda = -1\Rightarrow d_i = \frac{1}{\mu}+\frac{\lambda}{\mu}d_{i+1}.$$
	Using the above relation, we have $d_N=\frac{1}{\mu}$, $d_{N-1}=\frac{1}{\mu}(\frac{\lambda}{\mu})$, $d_{N-2}=\frac{1}{\mu}(\frac{\lambda}{\mu}+(\frac{\lambda}{\mu})^2)$, and
	$$d_1=\frac{1}{\mu}(\frac{\lambda}{\mu}+(\frac{\lambda}{\mu})^2+\dots+(\frac{\lambda}{\mu})^{N-1})=\frac{1-(\frac{\lambda}{\mu})^N}{\mu - \lambda}.$$
	Finally, we can write 
	\begin{align*}
	\mathbb{E}_N(\tau_0)=\sum_{k=1}^{N}d_k = \frac{N}{\mu-\lambda}+\lambda\frac{1-(\frac{\lambda}{\mu})^{N}}{(\mu-\lambda)^2}.
	\end{align*}
	\end{comment}
	Let $T_i$ denote the expected time for fully draining a queue containing $i$ requests. We have
	\begin{equation}(\mu+\lambda)T_{i}=1+\mu T_{i-1} + \lambda T_{i+1}, \quad i\in\{1,2,\ldots\}.
		\label{eq:recursive_mm1}
	\end{equation}
	We also have the boundary conditions $T_0 = 0$ and $\mu T_N = 1 + \mu T_{N-1}$.
	We can write
	\begin{equation*}
		\begin{cases}
			T_{i+1} - (\rho + 1)T_i + \rho T_{i-1}+\frac{1}{\lambda}=0\\
			T_{i} - (\rho + 1)T_{i-1} + \rho T_{i-2}+\frac{1}{\lambda}=0.
		\end{cases}
	\end{equation*}
	Subtracting the two equations above, we get
	$$T_{i+1} - (\rho+2)T_i + (2\rho+1)T_{i-1} - \rho T_{i-2}=0.$$
	For the above homogeneous difference equation, one can write the corresponding characteristic equation
	$$ z^3-(\rho+2)z^2 + (2\rho +1)z - \rho =(z-1)^2 (z-\rho),$$
	which has the set of roots $1, 1, \rho$. Thus, the solution to the recursive equation \eqref{eq:recursive_mm1} is given by
	\begin{equation*}
		T_i = 
		\begin{cases}
			(A+Bi) + C\rho^ i & \rho \neq 1\\
			A+Bi+C i^2 & \rho = 1,
		\end{cases}
	\end{equation*}
	where constants $A, B, C$ can be determined by applying the boundary conditions. These boundary conditions will give $A = 0$, $B = \left[\frac{1}{\mu} + \frac{2N-1}{2\lambda}\right]$, and $C = - \frac{1}{2\lambda}$ when $\rho = 1$. We also have 
	$C = -A = \left[\frac{\frac{1}{\mu} - \frac{1}{\lambda(\rho-1)}}{\rho^N - \rho^{N-1}}\right]$ and $B = \frac{1}{\lambda(\rho - 1)}$ when $\rho\neq 1$.
\end{proof}

==> python-code-basic-simulator.tex <==
\section{Full Python Code}
\begin{lstlisting}[language=Python]
import asyncio
import random

class Request:
    def __init__(self, client_id, request_id, future):
        self.client_id = client_id
        self.request_id = request_id
        self.future = future  # for response


class Server:
    def __init__(self, num_workers=3, process_time=1.0):
        self.queue = asyncio.Queue()
        self.process_time = process_time
        self.num_workers = num_workers
        self.worker_tasks = []
        self.running = False

    async def enqueue(self, request: Request):
        print(f"[Server] Enqueued request {request.request_id} from Client {request.client_id}")
        await self.queue.put(request)

    async def worker(self, worker_id: int):
        print(f"[Worker {worker_id}] Started.")
        while self.running:
            request = await self.queue.get()
            print(f"[Worker {worker_id}] Processing request {request.request_id} from Client {request.client_id}")
            await asyncio.sleep(self.process_time)
            if not request.future.done():
                request.future.set_result(f"Processed by worker {worker_id}")
            self.queue.task_done()
        print(f"[Worker {worker_id}] Exiting.")

    async def run(self):
        self.running = True
        self.worker_tasks = [
            asyncio.create_task(self.worker(i)) for i in range(self.num_workers)
        ]

    async def stop(self):
        self.running = False
        for _ in self.worker_tasks:
            await self.queue.put(Request(-1, -1, asyncio.get_event_loop().create_future()))
        await asyncio.gather(*self.worker_tasks)
        print("[Server] All workers stopped.")


class Client:
    def __init__(self, client_id, server: Server, retries=3, delay=1.0, timeout=2.0):
        self.client_id = client_id
        self.server = server
        self.retries = retries
        self.delay = delay
        self.timeout = timeout

    async def send_request(self, request_id):
        for attempt in range(1, self.retries + 1):
            future = asyncio.get_event_loop().create_future()
            req = Request(self.client_id, request_id, future)
            await self.server.enqueue(req)
            try:
                result = await asyncio.wait_for(future, timeout=self.timeout)
                print(f"[Client {self.client_id}] Request {request_id} succeeded: {result}")
                return
            except asyncio.TimeoutError:
                print(f"[Client {self.client_id}] Request {request_id} timed out (attempt {attempt})")
                await asyncio.sleep(self.delay)
        print(f"[Client {self.client_id}] Request {request_id} failed after {self.retries} retries")

    async def run(self, num_requests=5):
        for i in range(num_requests):
            await asyncio.sleep(random.uniform(0.1, 1.0))
            await self.send_request(i)


async def main():
    server = Server(num_workers=3, process_time=1.5)
    await server.run()

    clients = [Client(i, server) for i in range(3)]
    client_tasks = [asyncio.create_task(client.run()) for client in clients]

    await asyncio.gather(*client_tasks)
    await server.stop()

asyncio.run(main())
\end{lstlisting}
